Exceptional directions for the Teichm\"{u}ller geodesic flow and Hausdorff dimension

We prove that for every flat surface $\omega$, the Hausdorff dimension of the set of directions in which Teichm\"{u}ller geodesics starting from $\omega$ exhibit a definite amount of deviation from the correct limit in Birkhoff's and Oseledets' Theorems is strictly less than $1$. This theorem extends a result by Chaika and Eskin where they proved that such sets have measure $0$. We also prove that the Hausdorff dimension of the directions in which Teichm\"{u}ller geodesics diverge on average in a stratum is bounded above by $1/2$, strengthening a classical result due to Masur. Moreover, we show that the Hausdorff codimension of the set of non-weakly mixing IETs with permutation $(d, d-1, \dots, 1)$, where $d$ is an odd number, is exactly $1/2$ and strengthen a result by Avila and Leguil.

==> BirkhoffCorollary.tex <==
	\section{Dimension of Non-dense Orbits and Corollary~\ref{cor: Birkhoff corollary}}
    
    In this section, we outline how to deduce Corollary~\ref{cor: Birkhoff corollary} from the proof of Theorem~\ref{thrm: Birkhoff deviations thrm}.
    The idea is to translate all the results on horocycle arcs obtained in the previous sections to results on open bounded subsets of the strong unstable manifold for the Teichm\"{u}ller flow.
    For $\omega \in \mc{H}_1(\a)$, the strong unstable leaf of $\omega$, denoted by $\mc{W}^{su}(\omega)$ is defined by
    \begin{equation*}
    	\mc{W}^{su}(\omega) = \set{x\in \mc{H}_1(\a):  d_{\mc{H}_1(\a)}\left( g_t \omega, g_t x \right) \r 0 \text{ as } t \r -\infty }
    \end{equation*}
    where $d_{\mc{H}_1(\a)}$ denotes the Teichm\"{u}ller metric.
    
    
    Corollary~\ref{cor: Birkhoff corollary} is deduced from the following direct analogue of Theorem~\ref{thrm: Birkhoff deviations thrm}.
    \begin{theorem} \label{thrm: Birkhoff for unstable}
    Suppose $\mc{M}\subseteq \mc{H}_1(\a)$ is an affine invariant submanifold and $\nu_{\mc{M}}$ is the affine measure whose support is $\mc{M}$.
      Then, for any bounded continuous function $f$ on $\mc{M}$ and any $\e>0$, there exist affine invariant submanifolds $\mc{N}_1,\dots, \mc{N}_k$, properly contained in $\mc{M}$, and $\d >0$, such that for all $\omega \in \mc{M}\backslash \left( \cup_{i=1}^k \mc{N}_i \right)$,      
      the Hausdorff codimension of the set
      \begin{equation*}
          \set{x\in \mc{W}^{su}(\omega): \limsup_{T\r\infty} \left| \frac{1}{T} \int_0^T f(g_t x)\;dt -
                   \int_{\mathcal M} f \;d\nu_\mc{M}\right| \geqslant \e }
      \end{equation*}
      is at least $\d$.
    \end{theorem}
    
    
     
    {
    	\newcommand{\W}{\mc{W}^{su}}
        \newcommand{\Wl}{\mc{W}_{loc}^{su}}
    
    
    \subsection{Metrics and Measures on Unstable Leaves}
    Unstable leaves are immersed submanifolds and hence can be endowed with a metric coming from the restriction of $d_{\mc{H}_1(\a)}$. We denote such metrics by $\tilde{d}_{\mc{W}^{su}}$.
    Moreover, any such leaf is foliated with orbits of the horocycle flow $h_s$.
    In particular, we can locally find foliation charts for $h_s$-orbits within a leaf of the unstable foliation.
    We use $\Wl(\omega)$ to denote a neighborhood of a point $\omega$ inside $\W(\omega)$ which admits such a foliation chart.
    
    Foliation charts provide immersed local transversals for the horocycle orbits.
    We will use the notation $\mc{T}_\omega \subset \Wl(\omega)$ to denote a transversal of $h_s$-orbits given by some foliation chart on $\Wl(\omega)$.
    In particular, this gives a product structure of $\Wl(\w)$ as follows.
    \begin{equation*}
    	\Wl(\w) \ni x = h_{s(x)} t(x) \cong (t(x),s(x)) \in \mc{T}_\w \times I
    \end{equation*}
    where $I$ is an open interval and $(t(x),s(x))$ are determined uniquely by $x$ (and the choice of the chart).
    
    By restricting the metric $\tilde{d}_{\W}$ to a local transversal $\mc{T}_\w$, we obtain a metric on $\mc{T}_\omega$ which we denote by $d_{\mc{T}}$. We omit the dependence on $\w$ when it is clear from context.
    Thus, we can define a metric $d_{\Wl(\w)}$ on $\Wl(\w)$ as follows:
    \begin{equation} \label{metric on unstable chart}
    d_{\Wl(\w)} ( (t(x),s(x)), (t(y),s(y)) ) := \max\set{ d_{\mc{T}}(t(x),t(y)), |s(x)-s(y)| }
    \end{equation}
    for all $x,y \in \Wl(\w)$.
    
    
    
    
    By local disintegration of the Lebesgue volume measure on $\mc{H}_1(\a)$, one obtains a probability measure of Lebesgue class on small bounded  open sets of unstable leaves.
    These measures are denoted $\mu_{\mc{W}^{su}}$.
    Using the product structure on $\Wl(\w)$ (and assuming it is small enough so that $\mu_{\mc{W}^{su}}$ is defined),
    we can further disintegrate $\mu_{\mc{W}^{su}}$ as
    \begin{equation*}
    	d\mu_{\mc{W}^{su}}(t(x),s(x)) = ds\;d\mu_\mc{T}(t(x))
    \end{equation*}
    for some Lebesgue class measure on $\mc{T}$.
    
    Throughout this section, we fix a bounded continuous function $f$ on $\mc{H}_1(\a)$.
    We define analogous sets to those studied in Section~\ref{section: birkhoff}.
    For any positive $\e, N \in \mathbb R$, $M\in \N$ and a subset $Q \subseteq \mc{M}$, we define the following sets.
    \begin{align} \label{unstable B(f,N,epsilon,M)}
    	&\mf{B}_\omega (f, N, \e, M): = \set{x\in \Wl(\w): \frac{1}{MN}\int_0^{MN}f(g_tx) \;dt > \nu_{\mathcal M}(f) + \e  }\\
    	&\mf{Z}_\omega(Q, M, N, \e) := \set{ x\in \Wl(\w): 
        \frac{\#\set{0\leq i\leq M-1: g_{iN} x \notin Q} }{M} >\e }    \nonumber
   \\
   &\mf{B}_\omega (f, N, \e) := \limsup\limits_{M\r\infty} \mf{B}_\omega (f,N,\e,M) \qquad
    \mf{Z}_\omega(Q, N,\e) := \limsup_{M\r\infty}  \mf{Z}_\omega(Q, N,\e,M)  \nonumber
     \end{align}
     Next, for any $x\in \Wl(\w)$, $i\in \N$ and positive $\beta, N\in\mathbb R$, we define the corresponding functions and sets:
     \begin{equation} \label{unstable f_i}
       \mf{f}_i(x) := \frac{1}{N}\int_{iN}^{(i+1)N} f(g_tx) \;dt
       \end{equation}

       \begin{equation} \label{unstable F_i}
       		\mf{F}_i(\b) = \set{x\in \Wl(\w): \mf{f}_i(x) >  \nu_{\mc{M}}(f)+\b}
       \end{equation}
       
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \subsection{Sets and Partitions}
    Fix some $\w \in \mc{H}_1(\a)$.
    In this subsection, we define partitions of local unstable manifolds $\Wl(\w)$ analogously to those defined in Section~\ref{section: Birkhoff sets partitions}.
    Our partitions elements will have side lengths reflecting the rate of expansion under $g_t$.
    For this purpose, we define the following quantity. \todo{finite?}
    \begin{equation*} \label{eqn: side length}
    	\l(\w) :=  \sup \set{ \frac{ \log \norm{ D_x g_t(v) } }{t} :  x \in \Wl(\w), v\in T_x \mc{H}_1(\a), 
        \norm{v}=1, t>0  }
    \end{equation*}
    where $T_x \mc{H}_1(\a)$ is the tangent space at $x$, $D_x g_t$ is the derivative of the flow at $x$ and $\norm{\cdot}$ is the norm induced by the Teichm\"{u}ller metric.
    We note that $\l(\w)$ is finite and positive.
    In fact, $\l(\w) \geqslant 2$ since $g_t$ expands vectors tangent to the horocycle flow $h_s$ by a factor of $e^{2t}$.
    We suppress the dependence of $\l(\w)$ on $\Wl(\w)$ as it will be fixed in our arguments.
    
       
 		For $N,\eta >0$ and $i\in \N$, we define a partition $\mc{P}_{i,\eta}$ of $\Wl(\w)$ as follows.
        First, we choose a partition of the transversal $\mc{T}_\w$ into boxes of diameter at most $\eta e^{- \l(\w)iN/2 }$ (in the metric $d_\mc{T}$). We let $T_1,\dots, T_A$ be an enumeration of such a partition for some $A\in \N$.
        As for the horocycle direction, we recall the product structure $\Wl(\w) \cong \mc{T}_\w \times I$, where $I$ is an open bounded interval in $\R$.
        We partition $I$ into intervals of radius $e^{-2 iN}$ and let $J_1,\dots , J_B$ denote an enumeration of these intervals for some $B \in \N$.
        Finally, we define $\mc{P}_{i,\eta}$ to be
        \begin{equation*} \label{unstable P_i}
        	\mc{P}_{i,\eta} = \set{ T_a \times J_b: 1\leqslant a \leqslant A, 1\leqslant b \leqslant B}
        \end{equation*}
        where we view the boxes $T_a \times J_b$ as subsets of $\Wl(\w)$ under its identification with $\mc{T}_\w \times I$.
        
       For a set $Q \subset \mc{H}_1(\a)$, define the following sub-partitions
       \[ \mc{R}_{i,\eta}(Q) = \set{ B\in \mc{P}_{i,\eta}: \exists x\in B, g_{iN}x \in Q }  \]
          
    
    The following lemma is the analogue of Lemma~\ref{lemma: bad set for f and recurrent part of F_i} and its proof is identical so we omit it.
    Recall that $\mathcal{S}(f)$ denotes the Sobolev norm defined in~\eqref{eqn: sobolev norm upper bound}.
    \begin{lemma}
       	\label{lemma: bad set for f and recurrent part of F_i unstable}
        Suppose $Q \subset \mc{H}_1(\a)$. Then, for any $\omega \in \mc{H}_a(\a)$, $N,\e,\eta >0$, $0<\d \leq \frac{\e}{4 \mc{S}(f)}$, and $M\in \N$, 
        we have
            \[
            	\mf{B}_\omega (f,N,\e,M) \subseteq \mf{Z}_\omega(Q, M,N,\d) \cup 
                	\bigcup_{ \substack{ A \subseteq \set{0,\dots,M-1} \\
                				|A| = \lceil \d M \rceil } }
                                \bigcap_{i\in A}\mf{F}_i^{\mc{R}}(\e/2), 
            \]
         where $\mc{R}_{i,\eta} := \mc{R}_{i,\eta}(Q)$ for all $i\in \N$ and 
         \[
                        \mf{F}_i^{\mc{R}}(\e/2) = \mf{F}_i(\e/2) \cap \bigcup_{B\in \mc{R}_{i,\eta}} B. 
         \]
       \end{lemma}
       
       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    	\subsection{Measure Bounds}
        In this subsection, we show that the sets $\mf{F}_i$ can be made to have arbitrarily small measure proportion of any partition element inside $\mc{R}_{i,\eta}$ for an appropriate choice of $\eta$.
        This step is a direct analogue of Lemma~\ref{lemma: bound on measure of recurrent part of F_i} and relies on Theorem~\ref{thrm: quantitative Chaika-Eskin}
        \begin{lemma}
       \label{lemma: bound on measure of recurrent part of F_i unstable}
       For all $\ell >0$, there exists $\eta_0 >0$ so that for all $a >0$, there exists $T_0 >0$ such that 
       for all $N>T_0$, $\b>\e$, $i\in \N$, all $\omega \in \mc{H}_1(\a)$
       and all $B \in \mc{R}_{i,\eta_0}(C_\ell)$, we have
        \[ \frac{\mu_{\W} (B\cap \mf{F}_i(\b) )  }{\mu_{\W}(B)} \leqslant a,  \]
        where $\mu_{\W}$ is the Lebesgue probability measure on $\Wl(\w)$.
       \end{lemma}
    
    
    
    
    
    
    
    
    
    
    
    
    
    }
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
